Anonymity Unveiled: A Practical Framework for Auditing Data Use in Deep Learning Models

The rise of deep learning (DL) has led to a surging demand for training data, which incentivizes the creators of DL models to trawl through the Internet for training materials. Meanwhile, users often have limited control over whether their data (e.g., facial images) are used to train DL models without their consent, which has engendered pressing concerns. This work proposes MembershipTracker, a practical data auditing tool that can empower ordinary users to reliably detect the unauthorized use of their data in training DL models. We view data auditing through the lens of membership inference (MI). MembershipTracker consists of a lightweight data marking component to mark the target data with small and targeted changes, which can be strongly memorized by the model trained on them; and a specialized MI-based verification process to audit whether the model exhibits strong memorization on the target samples. MembershipTracker only requires the users to mark a small fraction of data (0.005% to 0.1% in proportion to the training set), and it enables the users to reliably detect the unauthorized use of their data (average 0% FPR@100% TPR). We show that MembershipTracker is highly effective across various settings, including industry-scale training on the full-size ImageNet-1k dataset. We finally evaluate MembershipTracker under multiple classes of countermeasures.

==> imagenet.tex <==

\label{sec:imagenet-exp}
This section evaluates \sysname under the full-sized ImageNet-1k training (over 1.28 million training samples). 
We train a ResNet50~\cite{he2016deep} and Swin-Transformer~\cite{liu2021Swin}, and they have 75.09\% and 80.29\% accuracy respectively (both with <1\% accuracy drop). 
We consider the challenging setting of supporting multiple users in different classes (1,000 target users in total). Each user contributes 125 samples to the training set, which is $<$0.01\% in proportion. 

We find that even under the large-scale training setting, the marked samples can still be strongly memorized by the models, which enables \sysname to achieve 0\% FPR@100\% TPR. % for all the users. 





Next, we evaluate how the performance varies with \emph{lesser} samples for marking (using ResNet50): we consider 63 and 32 samples by each user, which amount to $\sim0.005\%$ and $\sim0.0025\%$ of the training set. 
The results are in Fig.~\ref{fig:imagenet}.

\sysname can still maintain 0\% FPR@100\% TPR, when the marking ratio is reduced from 0.01\% to 0.005\%. 
However, when the marking ratio is further reduced to 0.0025\%, \sysname experiences lower auditing performance - 
this trend is similar to that in our ablation study in Appendix~\ref{sec:ablation-two-step-marking} and thus we defer the detailed discussion to Appendix~\ref{sec:ablation-two-step-marking} (due to space constraints). 
With that said, even under such a challenging case, \sysname still achieves reasonably good performance as shown in the blue line of Fig.~\ref{fig:imagenet}. %; we leave the improvements to future study. 
{
\emph{To the best of our knowledge, \sysname is the first technique that can scale to support reliable data auditing in large-scale training setting.}
}

\begin{figure}[t]
  \centering
  \includegraphics[ height=1.3in]{fig/imagenet.pdf}
  \caption{\sysname under full-sized ImageNet training with different portions of samples for data marking. 
  Aggressively reducing the portion of samples marked by each user can lead to reduced performance, though \sysname can still maintain reasonably high auditing performance even when each user can only mark merely 0.0025\% of the training data (the blue line). }
  \label{fig:imagenet} 
  \vspace{-3mm}
\end{figure}
